Do We Always Need the Simplicity Bias? Looking for Optimal Inductive Biases in the Wild

Neural architectures tend to fit their data with relatively simple functions. This "simplicity bias" is widely regarded as key to their success. This paper explores the limits of this principle. Building on recent findings that the simplicity bias stems from ReLU activations [96], we introduce a method to meta-learn new activation functions and inductive biases better suited to specific tasks. Findings: We identify multiple tasks where the simplicity bias is inadequate and ReLUs suboptimal. In these cases, we learn new activation functions that perform better by inducing a prior of higher complexity. Interestingly, these cases correspond to domains where neural networks have historically struggled: tabular data, regression tasks, cases of shortcut learning, and algorithmic grokking tasks. In comparison, the simplicity bias induced by ReLUs proves adequate on image tasks where the best learned activations are nearly identical to ReLUs and GeLUs. Implications: Contrary to popular belief, the simplicity bias of ReLU networks is not universally useful. It is near-optimal for image classification, but other inductive biases are sometimes preferable. We showed that activation functions can control these inductive biases, but future tailored architectures might provide further benefits. Advances are still needed to characterize a model's inductive biases beyond "complexity", and their adequacy with the data.

==> misc.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors

\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs} % for professional tables
\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage{floatrow}
\usepackage{sidecap}
\usepackage{subcaption}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage[title]{appendix}

% \newtheorem{theorem}{Theorem}[chapter]

\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\usepackage{cuted}
\setlength\stripsep{3pt plus 1pt minus 1pt}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}%[report]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\input{math_commands.tex}

\usepackage{url}            % simple URL typesetting
\usepackage{xcolor}         % colors
\usepackage{tikz,braket}
\usetikzlibrary{tikzmark,calc,shapes.geometric}
\usepackage[english]{babel}
\usepackage{amsthm,amsmath,amsfonts,amssymb}
\usepackage{mathrsfs}
%\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.
\usepackage{enumitem}

%\usepackage[hang,marginal]{footmisc} % No indentation of footnotes
\usepackage[percent]{overpic} % Overlay on image
\usepackage{bbm}
\usepackage{color,soul}
\usepackage{makecell}
\usepackage{tabularx,ragged2e}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\usepackage{mwe}
\usepackage{wrapfig}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{setspace}
\usepackage{array}
\newcolumntype{x}[1]{>{\centering\hspace{0pt}}p{#1}}
\usepackage{circledsteps}
\usepackage{extarrows}
\usepackage{graphbox}
\usepackage{comment}

% Caption on side of figure
\usepackage{xargs,caption,changepage,ifthen}
\newcommandx{\mycaptionminipage}[3][3=c,usedefault]{%
    \begin{minipage}[#3]{#1}%
        \ifthenelse{\equal{#3}{b}}{\captionsetup{aboveskip=0pt}}{}
        \ifthenelse{\equal{#3}{t}}{\captionsetup{belowskip=0pt}}{}
        \vspace{0pt}\centering\captionsetup{width=\textwidth} %Temporarily set caption width
        #2%
    \end{minipage}%
}%
\newcommandx{\mysidecaption}[4][4=c,usedefault]{%
    \mycaptionminipage{\dimexpr\linewidth-#1\linewidth-\intextsep\relax}{#3}[#4]%
    \hfill%
    \mycaptionminipage{#1\linewidth}{#2}[#4]%
}%

\definecolor{lightGray}{gray}{0.97}
\definecolor{midGray}{gray}{0.65}
\definecolor{lightYellow}{RGB}{254,254,242}

\mdfdefinestyle{citationFrame}{%
  linecolor=midGray,
  linewidth=0.5pt,
  roundcorner=3pt,
  skipabove=5pt,
  skipbelow=0pt,
  innertopmargin=3pt,
  innerbottommargin=3pt,
  innerrightmargin=5pt,
  innerleftmargin=5pt,
  leftmargin=0pt,
  rightmargin=0pt,
  backgroundcolor=lightGray
}

\mdfdefinestyle{yellowFrame}{%
  linecolor=midGray,
  linewidth=0.5pt,
  roundcorner=3pt,
  skipabove=6pt,
  skipbelow=3pt,
  innertopmargin=5pt,
  innerbottommargin=5pt,
  innerrightmargin=6pt,
  innerleftmargin=6pt,
  leftmargin=0pt,
  rightmargin=0pt,
  backgroundcolor=lightYellow
}

% No hyphenation
%\exhyphenpenalty=1000000
\hyphenation{mild}
\hyphenation{severe}
\hyphenation{distribution}
\hyphenation{shift}

% Short arrow
\usepackage{stmaryrd}
\usepackage{trimclip}
\makeatletter
\DeclareRobustCommand{\shortto}{%
  \mathrel{\mathpalette\short@to\relax}%
}
\newcommand{\short@to}[2]{%
  \mkern2mu
  \clipbox{{.5\width} 0 0 0}{$\m@th#1\vphantom{+}{\rightarrow}$}%
  }

% Long arrow
\makeatletter
\newcommand*{\da@rightarrow}{\mathchar"0\hexnumber@\symAMSa 4B }
\newcommand*{\da@leftarrow}{\mathchar"0\hexnumber@\symAMSa 4C }
\newcommand*{\xdashrightarrow}[2][]{%
  \mathrel{%
    \mathpalette{\da@xarrow{#1}{#2}{}\da@rightarrow{\,}{}}{}%
  }%
}
\newcommand*{\da@xarrow}[7]{%
  % #1: below
  % #2: above
  % #3: arrow left
  % #4: arrow right
  % #5: space left 
  % #6: space right
  % #7: math style 
  \sbox0{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#1#6\m@th$}%
  \sbox2{$\ifx#7\scriptstyle\scriptscriptstyle\else\scriptstyle\fi#5#2#6\m@th$}%
  \sbox4{$#7\dabar@\m@th$}%
  \dimen@=\wd0 %
  \ifdim\wd2 >\dimen@
    \dimen@=\wd2 %   
  \fi
  \count@=2 %
  \def\da@bars{\dabar@\dabar@}%
  \@whiledim\count@\wd4<\dimen@\do{%
    \advance\count@\@ne
    \expandafter\def\expandafter\da@bars\expandafter{%
      \da@bars
      \dabar@ 
    }%
  }%  
  \mathrel{#3}%
  \mathrel{%   
    \mathop{\da@bars}\limits
    \ifx\\#1\\%
    \else
      _{\copy0}%
    \fi
    \ifx\\#2\\%
    \else
      ^{\copy2}%
    \fi
  }%   
  \mathrel{#4}%
}
\makeatother

\renewcommand{\paragraph}[1]{\noindent{\normalsize\bfseries #1}\hspace{.05em}} % Bold paragraph titles

\def\bbE{\mathbb{E}}
\def\bbR{\mathbb{R}}
\def\bbP{\mathbb{P}}
\def\bbV{\mathbb{V}}
\def\cJ{\mathcal{J}}
\def\bx{\boldsymbol{x}}
\def\by{\boldsymbol{y}}
\def\bz{\boldsymbol{z}}
\def\bu{\boldsymbol{u}}
\def\bv{\boldsymbol{v}}
\def\bw{\boldsymbol{w}}
\def\bm{\boldsymbol{m}}
\def\bh{\boldsymbol{h}}

\def\bS{\boldsymbol{S}}
\def\bO{\boldsymbol{O}}
\def\bP{\boldsymbol{P}}
\def\bQ{\boldsymbol{Q}}
\def\bI{\boldsymbol{I}}
\def\bX{\boldsymbol{X}}
\def\bY{\boldsymbol{Y}}
\def\bZ{\boldsymbol{Z}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cU{\mathcal{U}}
\def\cW{\mathcal{W}}
\def\cV{\mathcal{W}}
\def\cI{\mathcal{I}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\newcommand{\bs}[1]{\boldsymbol{#1}}


==> sec/2e_others.tex <==
%----------------------------------------------------------------------------------------------------
\begin{comment}
\subsection{Value Estimation in Reinforcement Learning}
\label{sec:rl}

TODO.

Run on offline RL datasets (predict action given a state)
  run experiments from [1] while learning AFs -> find better AF than ReLU/sine
  [1] Frequency and Generalisation of Periodic Activation Functions in RL

\citet{mavor2024frequency} recently showed that sine activations in the critic help with sample efficiency, but not generalization.

\cite{lee2024simba}
show simplicity-biased architecture much better

\cite{farebrother2024stop}
histogram loss instead of MSE to learn value fct
\end{comment}

%----------------------------------------------------------------------------------------------------
\begin{comment}
\subsection{Studying Model Capacity}
Just How Flexible are Neural Networks in Practice: this paper shows significant differences of a given architecture in its capacity to overfit different tabular datasets
  we can explain this with the adequacy between architecture/dataset
  demonstration: repeat their experiment, then tailor the architecture to each dataset, and show that the differences vanish (= similar capacity across datasets when looking at matching pairs of architecture/dataset)

%----------------------------------------------------------------------------------------------------
\subsection{Demonstrate Practical Utility}

distill existing large model into shallow one with learned AF: trade off depth for width? (plot equi-performance curves for depth/width)
  need a case where a deep model is useful (clearly better than a shallow one)
  resnet -> resnet with fewer blocks?
  if not working: maybe means that *optimization* is still easier with deep network?
  apply to SOTA distillation method (paper by Beyers)

%----------------------------------------------------------------------------------------------------
\section{Analysis of Learned Activation Functions}
\label{sec:analysis}

Experiments on toy synthetic data
Serve as sanity check for the proposed experimental setup and method to learn AFs
learning AF
  on toy regression, linear/quadratic: learn the data-generating function
  (on parity task: learn the sine/sawtooth function)

REIMPLEMENT MULTIPLE ACT per (groups of) channels
explanation as "dictionary of wavelets" (Gaussian derivatives, Gabor filters = sine convolved with Gaussian)
= optimal space/frequency localization?
with multiple layers: never better if 1 layer large enough (?)
TODO train AF on Siemens star -> should learn Gabors of various frequencies; mask parts of the star -> limits range of Gabor activations learned?

\end{comment}


==> sec/trash.tex <==
%\title{Counterexamples to the Simplicity Bias: Learned Activation Functions\\Reveal the Adequacy Between Architectures and Data}
%\title{Counterexamples to the Simplicity Bias: Exploring the Adequacy\\Between Architectures and Data with  Learned Activation Functions}
%\title{Counterexamples to the Simplicity Bias:\\Exploring the Adequacy Between Architectures and Data}
%\title{Counterexamples to the Simplicity Bias:\\Is this Architecture Optimal for my Dataset?}


%The success of neural networks is often attributed to their ``simplicity bias''.
%by investigating how activation functions affect generalisation.
%we demonstrate benefits in controlling it
%this prior
%by meta-learning domain-specific activation functions.
%and demonstrate the importance of controlling this prior by meta-learning domain-dependent activation functions.

 %standard
%ReLU architectures are suboptimal


%Instead of hoping for a universal architecture, we should maybe look for identifying architectures that are best for a specific or a distribution of tasks.

%We discover that for many tasks, standard ReLU architectures are suboptimal.
%A prior for simplicity is often presented as universal, yet
%(not a single counterexample!)
%where the simplicity bias is suboptimal.

%We discover that for many tasks, standard ReLU architectures are suboptimal.
%Yet, our examples clearly link the success of neural networks to the

%Even though simplicity is often presented as universal prior, our examples clearly link the success of neural networks instead to the 
%\textbf{adequacy} between architectures and data.

%Tailored architectures may therefore remain useful.

%More broadly, the emergence of complex reasoning that requires postulates beyond the data may also not result from fitting observations with simplicity-biased architectures.


The remarkable generalization abilities of neural networks are often thought to originate from

This paper explores this adequacy between architectures and data,
and shows that the simplicity bias is ubiquitous but not universal.
generating the data.
encapsulated in principles such as Occam's razor.  or Solomonoff Induction.
This paper explores cases of \textbf{tasks} and \textbf{architectures} where this adequacy is broken.
This paper explores cases where this adequacy between architectures and data is broken.
and shows that the simplicity bias is ubiquitous but not universal.
We discover the optimal complexity level for a given task by meta-learning activation functions that provide the inductive biases with the best generalization for this task.
shift a network's prior towards a different level of complexity.
prior over functions specified primarily by the choice of activation function

across applications of machine learning

To study the adequacy between architectures and data, we introduce a method to meta-learn new activation functions, which are key to induce or alter the simplicity bias.

remarkable performance with low network depth (single wide hidden layer)
improved generalization on reasoning tasks and tabular datasets that neural networks typically struggle with.
explains why NNs struggle on some tasks (eg tabular data better handled by decision trees)
explains why certain architectures are particularly popular (relus, batch norm, ...)
on tabular datasets where boosted trees normally outperform NNs, this enables models with these learned AFs to match the performance of these trees

flat minima
    Explaining flat minimas with structure of parameter space
    hypothesis: flat minima = regions in parameter space that correspond well to the "default complexity" of the architecture
      e.g. for ReLU MLPs, means low complexity = often good generalization
      flat minima = solutions that rely on the "default spectrum"; for "simple" datasets, flatter = better
      sharp minima = solutions that rely on intricate combinations of weights to encode an "unusual" spectrum: for "complex" datasets, sharper = better
    key demonstration: flat minima are bad (worse than sharp ones) when the architecture/unductive biases mismatch the task
    related work
      "A modern look at the relationship between sharpness and generalization", Andriushchenko et al.
      they show that the "flat minima = better generalization" conjecture does not hold in general, even though often beneficial to move toward a locally flatter solution (SAM effective closer to the end of training)
      "Why are Sensitive Functions Hard for Transformers"
      complex functions (sensitive) are sharp minima; specific to transformers, theoretical + empirical, boolean functions only

--
Our technical novelty that allows new findings
  Optimization procedure \& parameterization of activation function that allow finding a good (global?) minimum with no bias/prior (can learn an arbitrary function, even complex/jagged)
Naive solutions for optimizing the act fct and why they fail
  at the end of training: does not take into account the training trajectory until then
  during training: cannot be applied from the start
  meta learning over whole inner training (with 2nd derivatives, differentiating the SGD training): too expensive for more than a few training iterations
  typical parameterizations: biased
Two technical difficulties
  Parametrization
    we don't want to introduce a bias (= be able to learn any "shape")
    our solution: interpolation (learn interpolation points, starting from constant/0 or random values)
  Optimization
    we could optimize it online like the weights, but an update of the activation function would also affect the prior optimization trajectory, hence the current state of the weights might have never been reached
    alternatively, would could use do meta learning (with 2nd order gradients) over the full optimization trajectory, but it is computationally difficult if we consider a long (full) training run
    simple version, only optimizing over a short training run: not good in practice
Our solution: mix of the 2 ideas
  initialize the activation function to constant 0
  with the current activation function
    do a short training run
    optimize the activation function with weights fixed
    increase the length of the training run
  repeat

Most work on learning activation function use a restrictive parametrization.
Typically, the activation function is implemented as a mini MLP~\cite{apicella2019simple}.
However this MLP itself needs an activation function, e.g.\ a ReLU, but then it has itself a simplicity bias, such that it will tend to learn a smooth function, which defeats the purpose of discovering really new functions.

Objective function to optimize the activation function: loss on training set, or (better) a validation set, or (even better?) on an OOD validation set

Major difference with all previous work on learning activation functions
  we don't train the act fct along the weights of the network (with a unique training objective) just like another set of parameters
  what we do: we train the weights and the act fct for different objectives (fitting tr data / generalizing to unseen or even OOD data)
  the goal is also different: we aim to train an activation function that captures the inductive biases useful for a range of tasks (meta learning setting) so that it can be reused across tasks

--

What our results show is that there also exist real-world learning tasks
that can benefit from different inductive biases.
Modern neural networks are undoubtedly remarkably effective across a variety of tasks.

But this is enabled by an assortment of design choices and architectural components (including activation functions) selected by trial and error specifically for this purpose,

Regardless, the message of this paper is valid but the title could have been ``\textit{Counterexamples to the inductive biases of ReLU-based architectures}''.
the suitability of an architecture for a dataset depends on

(or a data-generating function).
And there are multiple ways to measure it
(i.e.\ multiple proxies estimating the \textit{Kolmogorov complexity}, itself non-computable).
Future work on the adequacy between data/architecture should find ways to characterize  topic should 

Simplicity has also been used in the literature to refer to various 
is also ill-defined.
\textit{Kolmogorov complexity} is well defined
but it is non-computable and different proxies exist to approximate it.

--

%that is intuitive and relatively easy to characterize.
%which are difficult to fully characterize.
%We adopt this terminology because it is ubiquitous, but our study is more broadly relevant.
%is used loosely in the literature.
%Intuitively, a linear function is simple while a random walk is not.


%Theoretical results usually correspond to a 
 %simplicity 

are essential in inducing the simplicity bias
%are the main reason for the simplicity bias

%can be explained much more simply.
%independently from the training dynamics or even from the training data distribution. It
%is instead an intrinsic property of \emph{some} popular architectural choices,
%in particular ReLU-like activation functions.
%in particular that MLPs have strong inductive biases yet remain universal.
%present in untrained networks with certain architectures (e.g. ReLU MLPs, transformer LMs)

--
%of a typical neural architectures is
%for a variety of tasks and datasets. 
%\liang{not sure, but maybe we need to be careful on the terms `task' and `dataset' throughout the paper. Normally people would assume the optimal bias can be drastically different across tasks but only slightly different across datasets from a given task. Is it also the case in our conclusion, or should we add some clarification?}
%\liang{While the method can discover dataset-specific activation function, I am wondering if it's better to use `task' instead of `dataset' in the paper title because it aligns better with the intuition that different tasks would need different bias.}
%Our goal is to evaluate whether the simplicity bias is suitable or even optimal for specific tasks and datasets.
%Earlier work~\cite{teney2024neural} showed that the choice of activation functions is critical to induce the simplicity bias.


%that are sometimes completely unlike any existing one
%and that improve accuracy when the simplicity bias of standard ReLUs is not optimal.
%to enable the discovery of arbitrary activation functions that correspond to inductive biases very different from standard handcrafted architectures.

%learn an activation function from scratch
%the AF is encoded non-parametrically as a spline, this is key to avoid putting a prior on what the learned AF (which most existing work does, by parameterizing the AF as a small MLP for example, which has a smoothness prior)
%this allows learning the inductive biases of a neural network most suitable to enable (ID or OOD) generalization


%by learning new activation functions, optimized for generalization on a specific dataset.
%the simplicity bias
%is mainly due to
%mainly emerges in common architectures through
%the ubiquitous ReLU activations and their variants~\cite{hendrycks2016gaussian,ramachandran2017swish}.
%as rectified linear units (ReLUs) and their variants.
%Motivated by this finding, we build a new method
%to discovers optimal activation functions for any given dataset.

The \textit{spectral bias~}\cite{rahaman2019spectral}
and \textit{frequency principle}~\cite{xu2019frequency}
are closely related to the simplicity bias.
They refer to the observation that NNs learn low-frequency components of the target function earlier during training.
Works on this topic are specific to gradient descent
\cite{soudry2018implicit,xu2019training}.
and often to ReLU networks~\cite{hong2022activation,huh2021low,zhang2023shallow}.
--

%(see~\citet{mingard2023deep} for a review of the philosophical literature)
%It mirrors principles such Occam's razor and Solomonoff Induction.
%results in AIT (algorithmic information theory)
%So simplicity bias is a useful inductive bias.
%Yet we know that there is no universal inductive bias (NFL).
%This implicitly assumes that simple functions are \emph{always} best.
%It assumes that the underlying data-generating process in the real world are relatively simple,
%following the philosophical principle of Occam's razor.
%It implicitly 

--
OOD benchmarks: learn AF that focus on different features on waterbirds, CelebA (well-known datasets)
(Note: no issue with "cheating" if the goal is just to demonstrate that what is a shortcut/preferred feature is architecture-dependent)
  on synthetic staircase data from: 2024 Complexity Matters - Feature Learning in the Presence of Spurious Correlations
  Hypothesis why spectralNormalization hurts: makes the optimization of the network weights more difficult (additional constraint means more complex optimization trajectories)
    learning act fct *without spectralNormalization* can still be helpful because we saw in the redshift paper that the magnitude of the weights didn't change much during training anyway
    so if the act fct was optimized for the same initial weight magnitude as used when retraining, it should be appropriate

--
%\subsection{Shortcut Learning and Spurious Correlations}


\begin{comment}
Simplicity is only one %(ill-defined)
aspect of the inductive biases of NNs.
%which are difficult to fully characterize.
We adopt this terminology because it is ubiquitous, but our study is more broadly relevant.
%Our message is broader: what we show is the benefit of tweaking the inductive biases (in a general sense, not only along this one dimension)
A precise title could be
``\textit{Counterexamples to the inductive biases of ReLU-based architectures}''.
\end{comment}


%instead of the cross-entropy.
 %we comparing the ground truth class with the closest class ID to the model's output.
%The only difference is that the models now output a single scalar instead of class probabilities,
%and the regression objective 
%is to directly predict a class ID (each dataset contains 10 classes, and we assign each class a
%value in $[-1,1]$ as the regression target).
%We replace the classification task with a
%We create regression tasks where each of the 10 classes corresponds to a different value in $[-1,1]$.
%We then repeat the same experiments, except for


% References on sharpness
% 2021 Sharpness-Aware Minimization for Efficiently Improving Generalization (like Lipschitz or Jacobian regularization, wrt wts not input; finds wide loss valleys)
% 2017 Visualizing the loss landscape
% 2024 Sharpness-diversity tradeoff - improving flat ensembles with SharpBalance (less diversity in pred across models trained with SAM, ie fewer flat minima)
% 2023 Modern Look at the Relationship between Sharpness and Generalization (in transformers; inconsistent; flatter probably often better locally but not globally)

\begin{comment}
\paragraph{Dataset- vs.\ task-specific inductive biases.}
One could hope to transfer learned AFs across datasets of a same task.
But here we observed that different datasets require different inductive biases
Because "tabular datasets" is very non-specific. It just refers to low-dimensional inputs of disparate types, and there's just a huge variety of problems (and underlying data-generating processes) that match this description.
\end{comment}


\begin{comment}
\paragraph{A large variance across datasets}
shows up in the detailed results in 
\hyperref[sec:results2Tabular]{Appendix~\ref{sec:results2Tabular}}.
In some cases, ReLU MLPs work very well.
We explain this in 
\hyperref[fig:tabDim]{Figure~\ref{fig:tabPlots}}
by noting that the accuracy peaks, for some datasets, at the lowest complexity level.
In these cases, models with a strong simplicity bias
e.g.\ ReLU MLPs already do quite well.
The fact that different datasets require very different inductive biases is unsurprising.
``Tabular'' only refers to their low dimensionality, and these datasets have otherwise little in common.
\end{comment}

% \paragraph{When and why NNs generalize is yet to be understood.}
% Neural networks (NNs) have proven more effective than any other machine learning model.
% %\liang{However, they have failure modes and we need to understand when and why they generalize}
% %However we are still missing a complete explanation for
% %their ability to generalize across a variety of tasks and domains.
% However, they still have failure modes and we miss a complete explanation for their generalization abilities.
% A better understanding of this ability would help
% (1)~addressing these failure modes and (2)~better controlling or predicting their behavior.
% %with (1)~anticipating the successes and failures of neural models,
% %and (2)~addressing their many remaining limitations.
% Indeed, building neural networks is still an art based on trial and error.
% %that relies on trial-and-error and empirical evaluation.
% Understanding the conditions for generalization
% would enable the design of architectures, data collection, and data preparation
% procedures from first principles.
% Moreover, this understanding could help addressing failures to generalize %correctly
% %addressing neural networks have many remaining limitations
% %, some subtle and unforeseeable
% e.g.\ with shortcut learning~\cite{geirhos2020shortcut,teney2021evading},
% distribution shifts~\cite{jiang2024ood,teney2024id},
% biased data~\cite{gallegos2024bias},
% or compositional generalization~\cite{ren2024understanding,wiedemer2024compositional}.
% And these limitations are relevant even at the largest scales, such as
% with bias in RLHF~\cite{sun2024exploring},
% spurious correlations during in-context learning~\cite{harutyunyan2024context},
% or length generalization with large language models~\cite{anil2022exploring}, for example.

--
%Regression is another setting
%where we hypothesized that the inductive biases of ReLUs could be suboptimal.


%by discretizing the target~\cite{farebrother2024stop,imani2024investigating}.

%the inductive biases of typical ReLU architectures are not suitable.
%Regression tasks
%~\cite[Fig. 20]{grinsztajn2022tree}
%the simplicity bias of ReLU networks~\cite{dherin2022neural}.
%The intuition is that activations are more important for regression than classification
%since they determine the ``shape'' of the function implemented by a network.
%And this is particularly relevant since the scalar output of a regression model
%is used directly,
%whereas the output of a classification model is first discretized (logits turned into class IDs).


\florin{when comparing averages over different tasks we should normalize to some baseline because some tasks are more difficult than others and we don't want that to be lost in the average. Eg.: in Atari we normalize relative to the random policy and the human performance. In the ``Closing the gap...'' paper~\cite{dragoiclosing} we normalized relative to the random classifier (0.5 for all dsets) and the maximum performance ever achieved by a model on that task.}

\florin{I'm not sure I understand this argument in the current form. I assume the point of the paragraph is that while SGD can optimize towards simple or complex functions (as seen in the plots), the bias towards complex functions itself is not caused by SGD. However it's not obvious to me why is this the case. Just because some architectures converge to high complexity faster? This could still mean that SGD actually does have a bias towards simple functions that can be overcomed by a proper choice of activation function/architecture.}

%\florin{Higher level Q: Are the ReLU experiments having a comparable budget as the full meta-learning algo? One could argue that at least some of the differences we're seeing in generalization performance is due to the additional compute we put in sampling the function space. Eg.: would ReLU with warm restarts and a comparable budget would do better?}




\florin{when comparing averages over different tasks we should normalize to some baseline because some tasks are more difficult than others and we don't want that to be lost in the average. Eg.: in Atari we normalize relative to the random policy and the human performance. In the ``Closing the gap...'' paper~\cite{dragoiclosing} we normalized relative to the random classifier (0.5 for all dsets) and the maximum performance ever achieved by a model on that task.}


\liang{not sure if I understand the message of the following? I think people might get confused about why complexity bias is 'not' caused by 'optimization' since Figure 5b shows 'training trajectories/dynamics'}



%all models follow a continuous path of increasing complexity during training.
%But this increase is fastest for the best model (learned IAF).


%\paragraph{Learned activation function induces shaper complexity landscape.}



%In contrast to the first landscape figure that depicts a plane aligned with the
%While the global landscape depicts a plane aligned with the global
%training trajectory,
%(its two principal components),
%the zoom-in



%optimized model's



\liang{emph the tasks?}


%components in modern architectures and optimization schemes
%(e.g.\ Fourier embeddings~\cite{shi2024improved} which are equivalent to sine/cosine activations).
%other mechanisms (architectural, optimization) to modify inductive biases and reach complex solutions


%We only varied the activation function in minimal MLPs.
%But modern architectures include many components that shape their inductive biases.
%To measure the adequacy of these components with our methodology,

%One could define differentiable parametrizations of these components,
%then apply our meta learning approach to optimize them.
%This could determine whether a given architecture is best suited to a given dataset and possibly improve it.

%The proposed method should be applicable to any other task and could serve to improve state-of-the-art architectures.



%in the literature
%from philosophy~\cite[Appendix~A]{mingard2023deep}


%from philosophical writings (Occam's razor~\cite{})
%to recent discussions in AI~\cite{}.


%, with multiple ways to estimate it.
%Future work should seek other quantifiable properties to characterize them more fully.



%We learned dataset-specific activations
%because the goal was to discover optimal inductive biases. %for each dataset.
%But multiple similar datasets should benefit from these activations.
%One could even apply our meta-learning method on a 
%\emph{collection} of datasets (e.g.\ several tabular datasets)
%to discover general-purpose activations tuned for a particular domain,
%or for mitigating shortcut learning, for example.

%A first extension would be to use the suitability of learn activations across tasks to evaluate task similarity.


%to improve performance
%accuracy and training (convergence)
%in specific domains.
%on other sets of related tasks.



\begin{comment}
\paragraph{Limitations.}
\begin{itemize}[itemsep=1pt,topsep=0pt]
\item
Simplicity is \textbf{only one dimension}
to characterize inductive biases, with multiple ways to estimate it.
Future work should seek other quantifiable properties to characterize them more fully.

\item
We examined \textbf{minimal MLP architectures}
to isolate the effect of activations functions,
which are central to the simplicity bias~\cite{teney2024neural}.
But other components in modern architectures may already be tweaking or attenuating the simplicity bias (e.g.\ Fourier embeddings~\cite{shi2024improved} which are equivalent to sine/cosine activations).
\end{itemize}
\end{comment}


%reflects the importance of these tasks in the development of modern NNs.

%The proposed method could serve in the future to improve state-of-the-art architectures.

%be applicable to any other task and could serve 

%Even though simplicity is often presented as universal prior, our examples clearly link the success of neural networks instead to the \textbf{adequacy} between architectures and data.

%We also illuminate existing solutions that can be seen as special cases of our learned activations
%(e.g.\ Fourier features, periodic activation functions).
%\liang{The previous sentence is not clear to the reader, they will know what 'Fourier features and periodic activation functions' means but only after reading Sec 3.5 grokking, which is quite later}




% Option 1
%Neural architectures rely on various inductive biases to achieve generalization. ReLU activations are a popular choice known to bias learning toward simpler functions, resulting in strong generalization~\cite{teney2024neural}. However, in certain domains, such as tabular data, ReLU-based networks often fall short. In this paper, we explore whether alternative activation functions could enhance generalization, particularly in scenarios where conventional neural networks struggle to perform effectively.

% Option 2
%Neural architectures often prioritize learning simpler patterns. This tendency, known as \emph{simplicity bias}, is widely regarded as a cornerstone of their success. Commonly used ReLU activations have been shown to induce such simplicity bias~\cite{teney2024neural}. In this paper, we explore whether alternative activation functions could enhance generalization, particularly in scenarios where conventional neural networks struggle to perform effectively.

%Neural architectures often prioritize learning simple patterns.

%Common choices of architecture make neural networks fit data with simple functions.
%give neural networks a preference for fitting data with simple functions.
%This \emph{simplicity bias} is known as key to their success.

%optimal task-specific inductive biases.
%modulate this bias.
%It was demonstrated that different activation functions lead to neural networks with a simplicity bias of varying levels. This raises the question: is there a way to identify the optimal inductive biases from the data?



  %which is mainly driven by the choice of activation.
  %(Left)~We propose a method to discover new activations functions that improve generalization on specific datasets.
  %we find that the learned activation functions improve generalization on domains where standard simplicity bias is suboptimal by enforcing higher complexity prior.


---

%and results on individual datasets.

%The overall observation is that 
%the optimized activation functions (TanH with prefactor, learned AFs, and learned IAFs) perform better %than the ReLU baseline.

%fig:tabAllDatasets

%Our in-depth analyses focus on the \textsc{coverType} data because it has the largest training set and thus provides the most stable results.



\begin{comment}
  \citet{teney2024neural} showed that TanH activations with a prefactor could shift
  the simplicity bias towards a higher complexity by adjusting the prefactor to larger values.
    we evaluate the same MLPs with tanh and a prefactor (same on all layers; adjusting the LR to keep same optimization behaviour); prefactor in [.01 to 8], dimHidden 256
  results:
    could explain *some* cases where trees are better (tabCls 3: trees very good AND best prefactor very high), but not all
    makes sense: trees have other inductive biases (e.g. axis-aligned boundaries) that cannot be replicated by changing only the AF

test acc/complexity
    the best solutions require some precise level of complexity, \~similar level for different activation types (ReLU/tanh) = the simplest solutions are NOT the best ones
    (test acc/sharpness for comparison, there is no clear correlation, all over the place)

complexity/sharpness
    some correlation (different across activation types), well-tuned prefactor allows implementing complex functions that are less sharp = less rare in parameter space
    also true for learned AFs: this is why they work better: solutions with the right inductive biases (for the given dataset) are more common in the parameter space
    (SAM often fails to find flatter solutions: NEEDS sharp solution to implement complex functions to fit the tr data)
\end{comment}





\begin{comment}
\begin{mdframed}[style=citationFrame,userdefinedwidth=\linewidth,align=left,skipabove=6pt,skipbelow=0pt,innertopmargin=6pt,innerbottommargin=6pt]
\textbf{Notes on the sufficiency of shallow networks}\\[4pt]
  \textit{Understanding Deep Learning Requires Rethinking Generalization},~\citet{zhang2021understanding}\\[1pt]
  In this paper, Theorem 1 shows that a 1-layer ReLU network with $(2n\!+\!d)$ weights can fit any training set of $n$ examples (with data of dimension $d$).
    This shows that a single wide ReLU layer is enough to fit any training data, with a size proportional to number of training points.\\[5pt]
  \textit{Trading Positional Complexity vs.\ Deepness in Coordinate Networks}, \citet{zheng2022trading}\\[1pt]
  In this paper, Proposition 1 (Appendix A) shows that one can represent any function (i.e.\ fit any training set) with a hard-coded first layer (a.k.a.\ positional embedding)
  \textit{iff} the matrix of these positional embeddings for all training points is full-rank.
  In Section 5.1, they also show that a \textit{separable} positional embedding
  (which encodes each input dimension separately) is limited.
  This can only reconstruct a signal of rank $d$.
  This is quite intuitive: such a separable positional embedding can only represent a (coordinate-wise) separable signal.
  It means that one needs a \textit{deep} non-linear network (since depth adds rank)
  or a \textit{joint} positional encoding over all input dimensions.
  The latter is however quickly intractable for data of $>\!2$ dimensions.
\end{mdframed}

\clearpage
\begin{figure*}[ht!]
  \centering
  \includegraphics[width=.15\textwidth]{visualizations1/tabCls2_005.pdf} % complexity/sharpness
  \includegraphics[width=.15\textwidth]{visualizations1/tabCls2_004.pdf} % test acc/sharpness

  \includegraphics[width=.15\textwidth]{visualizations3/tabCls2_004.pdf} % Test acc / sharpness
  \includegraphics[width=.15\textwidth]{visualizations3/tabCls2_005.pdf} % Complexity / sharpness
    
  %Tanh with prefactor
  \includegraphics[width=.15\textwidth]{visualizations2/tabCls2_007.pdf} % Test acc / complexity

  \vspace{-8pt}
  \caption{\label{fig:tabAllDatasets2}
  TODO.
  }
\end{figure*}

\begin{mdframed}[style=citationFrame,userdefinedwidth=\linewidth,align=left,skipabove=6pt,skipbelow=0pt,innertopmargin=6pt,innerbottommargin=6pt]
\textbf{When are flat solutions beneficial?}\\[4pt]
   With the learned activation functions: we get more-complex models with less-sharp solutions.\\
    It has been noted before that whether flat-minima optimizers (e.g. sharpness-aware minimization, SAM) improves or worses generalization is dataset dependent (When Do Flat Minima Optimizers Work)
    Our observations suggest that flatness means that a model is close to the architecture's default level of complexity; whether this is a good thing depends on the adequacy between the architecture and task/dataset.

    Flatter solutions usually are more simple; whether this is beneficial for generalization depends on the task/dataset.
\end{mdframed}

\end{comment}





%Learning channel-specific non-linear transformations, then simple MLP on top: often even better than learning AF in hidden layers.
%Note: IAFs could be implemented as 1D-1D MLP with a learned, channel-specific activation)

%It's like learning a nonlinear transformation on each individual input.
%This is not surprising: tabular datasets are known to require little feature interaction

%the purported properties of tabular data such as low-order and sparse feature interactions
%These include Deep & Cross Networks (Wang et al. 2017),
%Wide & Deep Networks (Cheng et al. 2016),
%TabNets (Arik and Pfister 2019),
%and AdaNet (Cortes et al. 2016).

%(shown with tabFPN?? or a follow up where they train on synthetic data with no feature interactions?)



\begin{comment}
(1)\;Contrary to common belief, the simplicity bias is not universally useful.
Diverse real tasks benefit from different inductive biases.
%There exist diverse real tasks where
%it is suboptimal.
%(2)\;The suitability of ReLU models for image classification is not accidental.
%(2)\;The popularity of ReLUs originates in their success for image classification, but does not mean that they are always optimal.
(2)\;ReLUs are near-optimal for image classification, but this success does not mean that
they are the best choice for every task.
(3)\;The success of machine learning
hinges on the adequacy between data and architectures.
Therefore we might still find benefits in architectures tailored to specific (distributions of) tasks.
\end{comment}


